BuSCOPE : Fusing Individual & Aggregated Mobility Behavior for "Live" Smart City Services

While analysis of urban commuting data has a long and demonstrated history of providing useful insights into human mobility behavior, such analysis has been performed largely in offline fashion and to aid medium-to-long term urban planning. In this work, we demonstrate the power of applying predictive analytics on real-time mobility data, specifically the smart-card generated trip data of millions of public bus commuters in Singapore, to create two novel and "live" smart city services. The key analytical novelty in our work lies in combining two aspects of urban mobility: (a) conformity: which reflects the predictability in the aggregated flow of commuters along bus routes, and (b) regularity: which captures the repeated trip patterns of each individual commuter. We demonstrate that the fusion of these two measures of behavior can be performed at city-scale using our BuScope platform, and can be used to create two innovative smart city applications. The Last-Mile Demand Generator provides O(mins) lookahead into the number of disembarking passengers at neighborhood bus stops; it achieves over 85% accuracy in predicting such disembarkations by an ingenious combination of individual-level regularity with aggregate-level conformity. By moving driverless vehicles proactively to match this predicted demand, we can reduce wait times for disembarking passengers by over 75%. Independently, the Neighborhood Event Detector uses outlier measures of currently operating buses to detect and spatiotemporally localize dynamic urban events, as much as 1.5 hours in advance, with a localization error of 450 meters.

==> 4b.mod.tex <==
\section{Mobility On-demand Vehicles for Last-Mile Transport} 
\label{sec:disembarkation}

\begin{figure}[tbh]
\begin{center}
\includegraphics[scale=0.6]{pictures/placeholder.png}
    \caption{TBD XXX: disembarkation prediction accuracy vs. spatial quantization}
\label{fig:accuracyvsquantization}
\end{center}
\end{figure}



\begin{figure}[!htb]
\vspace{-0.2in}
  \centering
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=3in,height=2.3in]{pictures/2013-08-21_S1.jpg}
    \caption{Waiting time vs. resource utilization with strategy 1.}
    \label{fig:strategy1}
  \end{minipage}% 
  \hfill
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=3in,height=2.3in]{pictures/placeholder.png}
    \caption{Waiting time vs. resource utilization with strategy 2.}
    \label{fig:strategy2}
  \end{minipage}
\end{figure}

Figure~\ref{fig:strategy1}

\kas{todo: (1) can easily extend to all subzones, (2) if I can have a more ``representative" travel time instead}

==> 5.Ridership.tex <==
\subsection{On boarding Ridership Prediction}\label{sec:disembarkationprediction}
For each one of the trips, we sorted the data in the order of boarding time to the bus and simulated the boarding and alighting from bus stop to bus stop. In order to do this simulation we used a methodology as described by Figure \ref{fig:journeyreconstruction}. 
If the bus stops in a route X is denoted by the sequance $x_{0}, x_{1}, x_{2}, .... x_{n-1}, x_{n}$, we would have 2 arrays of n integers initialized to 0. One of these arrays is to simulate the real boarding alighting patterns and the other one would be used to simulate behavior of our predictions. Lets name these arrays $simulation_{actual}$ and $simulation_{predicted}$ respectively. For a traveler whose boarding bus stop is $x_{b}$, real alighting bus stop is $x_{a}$ \& predicted alighting bus stop is $x_{p}$; our model would add 1 to the b$^{\textnormal{th}}$ element of both $simulation_{actual}$ and $simulation_{predicted}$ arrays. Then 1 would be deducted from a$^{\textnormal{th}}$ element of $simulation_{actual}$ and p$^{\textnormal{th}}$ element of $simulation_{predicted}$. This addition and deduction in the two arrays denotes the boarding and alighting of users from the bus. 

At any time of the trip, if we want to find the predicted occupancy at a particular upcoming bus stop $x_{uc}$, we can use the  $simulation_{predicted}$ array and get the sum of elements till the uc$^{\textnormal{th}}$ elements. Similarly, we can use the array $simulation_{actual}$ to find the number of people who are actually in the bus during any time of the trip. At the end of a trip or during any time instance during the trip, if the i$^{th}$ element of $simulation_{actual}$ is denoted by $SA_i$, the i$^{th}$ element of $simulation_{predicted}$ is denoted by $SP_i$ and the number of stops within the route is \textit{n}, then the predicted occupancy for a particular bus stop is denoted as in equation \ref{eq:10} and the occupancy error at a particular bus stop and average occupancy error for a bus trip are given by \ref{eq:11} and \ref{eq:12} respectively. 

Using the above methodology, we were able to reconstruct bus trips and calculate the difference between real occupancy and predicted occupancy of a unique trip of a bus during the whole trip in each of the bus stops. We aggregated these occupancy error values for weekends and weekdays for all the services as shown in Figure \ref{fig:journeyreconstruction} in which the minimum average occupancy error for each service was obtained after calculating the errors for varying $N_{threshold}$ values as in Figure \ref{fig:journeyreconstruction}. It was observed that for 99.39\% of trips out of 6955 trips we considered in our experiment, the minimum error was observed when $N_{threshold}$=0 which is using the full personification in our hybrid approach. The accuracy of these reconstructions are really high in the sense, for CBD buses in weekdays, we were able to predict the number of people in a bus at a particular bus stop to an error of just 0.56 persons and for weekends it was a mere 1.73 persons. 

\begin{equation}\label{eq:10}
   \text{ Predicted Occupancy at P$^{th}$ bus stop = } \sum_{i=1}^{P} SP_i
\end{equation}

\begin{equation}\label{eq:11}
   \text{ Occupancy Error at P$^{th}$ bus stop = }\Big| \sum_{i=1}^{P} SA_i - \sum_{i=1}^{P} SP_i \Big|\
\end{equation}


\begin{equation}\label{eq:12}
   \text{ Average Occupancy Error for a trip = }\frac{\sum_{i=1}^{n} \Big| \sum_{i=1}^{n} SA_i - \sum_{i=1}^{n} SP_i \Big| }{n}
\end{equation}


\begin{figure}
  \includegraphics[width=0.49\textwidth]{pictures/RealVsPredicted.png}
  \caption{Journey Reconstruction Algorithm \& Ridership Prediction}
  \label{fig:journeyreconstruction}
\end{figure}


\begin{figure}
  \includegraphics[width=0.49\textwidth]{pictures/OccupancyResultsV2.png}
  \caption{Journey Reconstruction Algorithm \& Ridership Prediction}
  \label{fig:journeyreconstruction}
\end{figure}


\begin{figure}
  \includegraphics[width=0.49\textwidth]{pictures/OccupancyResultsSummaryV2.png}
  \caption{Journey Reconstruction Algorithm \& Ridership Prediction}
  \label{fig:occupancyerrors}
\end{figure}

\begin{figure}
  \includegraphics[width=0.49\textwidth]{pictures/JourneyReconstruction.PNG}
  \caption{Journey Reconstruction Algorithm \& Ridership Prediction}
  \label{fig:occupancyerrortypes}
\end{figure}

\subsection{Lookahead Time of Prediction}
According to the results we have obtained, our model is capable of predicting a disembarkation accurately before xx.xx bus stops in advance. In terms of time and distance, it is ~2.6km or 13 minutes of travelling time in advance. 

%\am{Add in results of how far in advance one can predict, and with what error.}

\subsection{Dynamic Occupancy Prediction Re-Adjustment}
The model we used provides highly accurate results for occupancy prediction as shown above in Figure \ref{fig:journeyreconstruction}, Figure \ref{fig:occupancyerrors} and Figure \ref{fig:occupancyerrortypes}. The above algorithm is a greedy algorithm in the sense, it doesn't re-adjust the results based on the real levels of occupancy in the bus and it's deviation from the predicted occupancy levels. Since the use case of our model is in real-time bus disembarkation analysis, we did an optimization to the simulation algorithm (mentioned in section \ref{sec:disembarkationprediction}) such that the model would learn from inaccurate predictions during the journey and re-adjust the predicted occupancy for all the upcoming bus stops. This \textit{Dynamic Prediction Re-Adjustment Algorithm} works in two stages depending on the nature of the journey. 
\\Step 1 - If the user has alighted before the predicted bus stop: In this case, the algorithm would adjust the predicted occupancy for the upcoming bus stops by reducing the predicted occupancy by 1. 
\\Step 2 - If the predicted bus stop has already passed for the specific user: In this case, depending on the original boarding bus stop, the algorithm would consider the possible alighting bus stops ranked in terms of confidence and choose the destination with highest confidence given that bus stop has not been already surpassed by the bus at that particular moment.

This dynamic model provides 2 main advantages according to our evaluations. (a) It gives our model the capability to switch to lower confidence alternatives instead of the higher confidence choice, and hence, increases the Average Overall Accuracy of our model from 86.17\% (as mentioned in Table \ref{tab:accuracyresults}) to 89.37\% with re-adjustments. This increase corresponds to correct predictions with multiple re-adjustments as well. (b) The dynamic model avoids the propagation of ridership prediction errors to the upcoming bus stops. In cases where the user has already alighted when the initial prediction is for an upcoming bus stop, dynamic model avoids the error propagation and results in highly accurate ridership predictions. 

%\am{Here explain the algorithm where the disembarkation is adjusted dynamically after each stop (once we see who has alighted or boarded), then provide some examples [including visual graphs] where looking at occupancy even 2-3 stops (as is commonplace today) in advance is misleading}

